Taxonomy Induction using Hypernym Subsequences

We propose a novel, semi-supervised approach towards domain taxonomy induction from an input vocabulary of seed terms. Unlike all previous approaches, which typically extract direct hypernym edges for terms, our approach utilizes a novel probabilistic framework to extract hypernym subsequences. Taxonomy induction from extracted subsequences is cast as an instance of the minimumcost flow problem on a carefully designed directed graph. Through experiments, we demonstrate that our approach outperforms stateof- the-art taxonomy induction approaches across four languages. Importantly, we also show that our approach is robust to the presence of noise in the input vocabulary. To the best of our knowledge, no previous approaches have been empirically proven to manifest noise-robustness in the input vocabulary.

==> figures/taxonomy-fig_original.tex <==
\begin{figure*}[t]
\begin{minipage}{0.8\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto]
  \tikzset{Category/.style ={shape=circle,fill=white,draw=black,minimum size=6mm,inner sep=0pt}}
  \tikzset{Discarded/.style ={shape=circle,fill=gray!50,draw=black,minimum size=6mm,inner sep=0pt}}
  \tikzset{Discarded2/.style ={shape=circle,fill=gray!5,draw=black,minimum size=6mm,inner sep=0pt}}
  \tikzset{Entity/.style ={shape=circle,fill=black,draw=black,text=white,minimum size=6mm,inner sep=0pt}}
  \tikzset{Name/.style = {text=black, node distance=4mm, align=center, scale=0.7, font=\relsize{0.7}}}
  \newcommand\NameW[2]{%
	\node[Name, left of=#1, anchor=east] (#1_t) {#2};
  }
  \newcommand\NameE[2]{%
	\node[Name, right of=#1, anchor=west] (#1_t) {#2};
  }
  \newcommand\NameNE[2]{%
	\node[Name, right of=#1, anchor=south west] (#1_t) {#2};
  }
  \newcommand\NameS[2]{%
	\node[Name, below of=#1, anchor=north, node distance=4mm] (#1_t) {#2};
  }
  \newcommand\NameN[2]{%
	\node[Name, above of=#1, anchor=south, node distance=4mm] (#1_t) {#2};
  }
  \newcommand{\EdgeSolid}[2]{%
  \draw [->] (#1) -- (#2);
  }
  \newcommand{\EdgeStyle}[3]{%
    \path[#3] (#1) edge (#2);
  %\draw [->] (#1) to [#3] (#2);
  }
  \newcommand{\EdgeDotted}[2]{%
  \draw [dotted,->] (#1) -- (#2);
  }

\begin{scope}[shift={(-4.9,-1.0)}]
   \node (group_a)	at (1.5, -1.4) {\large(a) Initial taxonomy};
   \node[Discarded]    (apple)	at (0, -0.2) {};
   \node[Discarded]  (orange)		at (2, -0.2) {};
   \node[Category]  (fruit)	at (1, 1.5) {};
   \node[Discarded2]  (food)	at (1, 3) {};
   \node[Discarded]  (spain)	at (3, 1) {};
   
    \NameW{apple}{\\ apple}
    \NameW{orange}{\\orange}
    \NameE{fruit}{\\ fruit}
    \NameW{food}{\\ food}
    \NameW{spain}{\\ Spain}
       
       \begin{scope}[every path/.style={->}, every node/.style={sloped, inner sep=1pt}]
 \draw (apple) -- node [anchor=north] {{\small 0.5}} (fruit);
 \draw (apple) -- node [anchor=south, pos=0.7] {{\small 0.2}} (food);
 \draw (orange) -- node [anchor=south] {{\small $0.5$}} (fruit);
 \draw (spain) -- node [anchor=south] {{\small $0.25$}} (food);
 \draw (fruit) -- node [anchor=north] {{\small $1$}} (food);
 \end{scope}
  \end{scope}
 
 
 
 
 \begin{scope}[shift={(0,-1.0)}]
   \node (group_b)	at (1.5, -1.4) {\large(b): Construction of the directed graph $G$};
   \node[Entity]    (start)	at (3.2, -1) {};
   \node[Entity]    (end)	at (1, 4.5) {};
   \node[Discarded]    (apple)	at (0, -0.2) {};
   \node[Discarded]  (orange)		at (2, -0.2) {};
   \node[Category]  (fruit)	at (1, 1.5) {};
   \node[Discarded2]  (food)	at (1, 3) {};
   \node[Discarded]  (spain)	at (3, 1) {};
   
    \NameW{start}{\\ start}
    \NameW{end}{\\ end}
    \NameW{apple}{\\ apple}
    \NameW{orange}{\\orange}
    \NameE{fruit}{\\ fruit}
    \NameW{food}{\\ food}
    \NameW{spain}{\\ Spain}
       
       \begin{scope}[every path/.style={->}, every node/.style={sloped, inner sep=1pt}]
 \draw (apple) -- node [anchor=north] {{\small (1, 2)}} (fruit);
 \draw (apple) -- node [anchor=south, pos=0.7] {{\small (1, 5)}} (food);
 \draw (orange) -- node [anchor=south] {{\small (1, 2)}} (fruit);
 \draw (spain) -- node [anchor=south] {{\small (1, 4)}} (food);
 \draw (fruit) -- node [anchor=north] {{\small (2, 1)}} (food);
 \end{scope}
  
 \begin{scope}[every path/.style={->, dashed}, every node/.style={sloped, inner sep=1pt}]
 \draw (start) -- node [anchor=north] {{\small (1, 1)}} (apple);
 \draw (start) -- node [anchor=south] {{\small (1, 1)}} (orange);
 \draw (start) -- node [anchor=south] {{\small (1, 1)}} (spain);
 \draw (food) -- node [anchor=south] {{\small (3, 1)}} (end);
  \end{scope}
 
 
 
 \end{scope}
 
 
 
 \begin{scope}[shift={(4.9,-1.0)}]
   \node (group_c)	at (1.5, -1.4) {\large(c): flow values for each  edge found using demand $d=3$};
   \node[Entity]    (start)	at (3.2, -1) {};
   \node[Entity]    (end)	at (1, 4.5) {};
   \node[Discarded]    (apple)	at (0, -0.2) {};
   \node[Discarded]  (orange)		at (2, -0.2) {};
   \node[Category]  (fruit)	at (1, 1.5) {};
   \node[Discarded2]  (food)	at (1, 3) {};
   \node[Discarded]  (spain)	at (3, 1) {};
   
    \NameW{start}{\\ start}
    \NameW{end}{\\ end}
    \NameW{apple}{\\ apple}
    \NameW{orange}{\\orange}
    \NameE{fruit}{\\ fruit}
    \NameW{food}{\\ food}
    \NameW{spain}{\\ Spain}
       
       \begin{scope}[every path/.style={->}, every node/.style={sloped, inner sep=1pt}]
 \draw (apple) -- node [anchor=south] {1} (fruit);
 \draw (orange) -- node [anchor=south] {1} (fruit);
 \draw (spain) -- node [anchor=south] {1} (food);
 \draw (fruit) -- node [anchor=north] {2} (food);
 \end{scope}
 
 \begin{scope}[every path/.style={->, dashed}, every node/.style={sloped, inner sep=1pt}]
 \draw (start) -- node [anchor=north] {1} (apple);
 \draw (start) -- node [anchor=south] {1} (orange);
 \draw (start) -- node [anchor=south] {1} (spain);
 \draw (food) -- node [anchor=south] {3} (end);
  \end{scope}
    \end{scope}
  
  
   \begin{scope}[shift={(9.8,-1.0)}]
   \node (group_d)	at (1.5, -1.4) {\large (d):  flow values for each  edge found using demand $d=2$};
   \node[Entity]    (start)	at (3.2, -1) {};
   \node[Entity]    (end)	at (1, 4.5) {};
   \node[Discarded]    (apple)	at (0, -0.2) {};
   \node[Discarded]  (orange)		at (2, -0.2) {};
   \node[Category]  (fruit)	at (1, 1.5) {};
   \node[Discarded2]  (food)	at (1, 3) {};
   \node[Discarded]  (spain)	at (3, 1) {};
   
    \NameW{start}{\\ start}
    \NameW{end}{\\ end}
    \NameW{apple}{\\ apple}
    \NameW{orange}{\\orange}
    \NameE{fruit}{\\ fruit}
    \NameW{food}{\\ food}
    \NameW{spain}{\\ Spain}
       
       \begin{scope}[every path/.style={->}, every node/.style={sloped, inner sep=1pt}]
 \draw (apple) -- node [anchor=south] {1} (fruit);
% \draw (spain) -- node [anchor=south] {0} (food);
 \draw (orange) -- node [anchor=south] {1} (fruit);
 \draw (fruit) -- node [anchor=north] {2} (food);
 \end{scope}
 
 \begin{scope}[every path/.style={->, dashed}, every node/.style={sloped, inner sep=1pt}]
 \draw (start) -- node [anchor=north] {1} (apple);
 \draw (start) -- node [anchor=south] {1} (orange);
 \draw (food) -- node [anchor=south] {2} (end);
 %\draw (start) -- node [anchor=south] {0} (spain);
  \end{scope}
    \end{scope}
    %\NameW{living}{Living \\ People}
    %\NameW{status}{People \\ by \\ status}
    %\NameW{people}{People}
	%\NameE{birth}{1962 \\ births};
	%\NameE{male}{Male actors \\ from NY};
	%\NameS{actors}{Actors};
	%\NameN{list}{Wikipedia \\  article list};
    
    %\EdgeSolid{cruise}{male};
    %\EdgeSolid{cruise}{tom};
    %\EdgeSolid{cruise}{living};
    %\EdgeSolid{cruise}{birth};
    %\EdgeStyle{male}{actors}{bend left};
    %\EdgeStyle{status}{people}{bend left};
    %\EdgeSolid{living}{status};
    %\EdgeSolid{living}{list};
    %\EdgeStyle{actors}{people}{dashed,bend right};    


%\begin{scope}[shift={(0,0)}]
%   \node (group_b)	at (-1.4, 3.8) 
%   {\large\textbf{(b)}};
%   \node[Entity]    (cruise)	at (1.2, 1.0) {};
%   \node[Discarded]  (male)		at (1.2, 2.0) {};
%   \node[Category]  (living)	at (0.3, 1.7) {};
%   \node[Category]  (actors)	at (1.2, 3.0) {};
%   \node[Discarded]  (status)	at (0.3, 2.7) {};
%   \node[Category]  (people)	at (0.3, 3.7) {};
   
%    \NameE{cruise}{\\ Tom \\Cruise}
%    \NameW{living}{Living \\ People}
%    \NameW{status}{People \\ by status}
%    \NameW{people}{People}%
%	\NameE{male}{Male \\ actors \\ from NY};%
%	\NameE{actors}{Actors};
    
%    \EdgeSolid{cruise}{male};
%    \EdgeSolid{cruise}{living};
%    \EdgeSolid{male}{actors};
%    \EdgeSolid{status}{people};
%    \EdgeSolid{living}{status};
%    \EdgeStyle{actors}{people}{dashed};    
%\end{scope}

%\begin{scope}[shift={(0.0,-1.4)}]
%   \node (group_c)	at (-1.4, 1.8) 
%{\large\textbf{(c)}};
%   \node[Entity]    (cruise)	at (1.2, 0.0) {};
%   \node[Category]  (living)	at (0.3, 0.7) {};
%   \node[Category]  (actors)	at (1.2, 1.0) {};
%   \node[Category]  (people)	at (0.3, 1.7) {};
   
%    \NameE{cruise}{\\ Tom \\Cruise}
%    \NameW{living}{Living \\ People}
%    \NameW{people}{People}%
%	\NameE{actors}{Actors};
    
%    \EdgeSolid{cruise}{actors};
%    \EdgeSolid{cruise}{living};
%    \EdgeSolid{living}{people};
%    \EdgeStyle{actors}{people}{dashed};    
%    \end{scope}
\end{tikzpicture}
}
%   \caption{ Minimum-cost flow algorithm for taxonomy induction. Fig.(a) shows the initial taxonomy with \textit{support} values for edges, three seed terms (\textit{apple}, \textit{orange} and \textit{Spain}), and the root \textit{food}. Fig.(b) shows the corresponding graph with (capacity, cost) values for each edge. Fig.(c) and (d) show the flow values for each edge found using demand $d = 3$ and $d=2$ respectively. Final taxonomy is the collection of all edges (excluding start and end nodes) with flow $>0$.}
  \caption{Execution of the minimum cost flow starting from our initial taxonomy}
  \label{fig:taxonomy-induction}
 \end{minipage}
 
\end{figure*}

